Entanglement Swapping in Quantum Switches: Protocol Design and Stability Analysis

Quantum switches are critical components in quantum networks, distributing maximally entangled pairs among end nodes by entanglement swapping. In this work, we design protocols that schedule entanglement swapping operations in quantum switches. Entanglement requests randomly arrive at the switch, and the goal of an entanglement swapping protocol is to stabilize the quantum switch so that the number of unfinished entanglement requests is bounded with a high probability. We determine the capacity region for the rates of entanglement requests and develop entanglement swapping protocols to stabilize the switch. Among these protocols, the on-demand protocols are not only computationally efficient, but also achieve high fidelity and low latency demonstrated by results obtained using a quantum network discrete event simulator.

==> LatexInclusion/Acronym-Def.tex <==
%----------------------------------------------------------------------------------------------------------------------%
%                    U s e r  -- D e f i n e d   S e l f  --  e x p a n s i o n  A c r o n y m s                   %
%----------------------------------------------------------------------------------------------------------------------%

\usepackage{acronym}
\acrodef{uwb}[UWB]{ultra-wideband}
\acrodef{fy}[FY]{fiscal year}

\acrodef{iot}[IoT] {Internet of Things}
\newacro{aws}[AWS]{Amazon Web Services}

\acrodef{ble}[BLE]{Bluetooth Low Energy}

\newacro{dfe}[DFE]{decision feedback equalizer}
\newacro{lms}[LMS]{least means square}
\newacro{ann}[ANN]{artificial neural network}
\newacro{alu}[ALU]{arithmetic logic unit}
\newacro{api}[API]{application programming interface}
\newacro{asic}[ASIC]{application-specific integrated circuit}

\newacro{sdn}[SDN]{software defined network}
\newacro{hca}[HCA]{heterogeneous computing architecture}


\acrodef{gps}[GPS]{Global Positioning System}
\acrodef{imu}[IMU]{inertial measurement unit}
\acrodef{uav}[UAV]{unmanned aerial vehicles}


\acrodef{csi}[CSI]{channel state information}
\acrodef{snr}[SNR]{signal-noise-ratio}


\acrodef{los}[LOS]{line-of-sight}
\acrodef{nlos}[NLOS]{non-line-of-sight}
\newacro{toa}[TOA]{time-of-arrival}
\newacro{tdoa}[TDOA]{time-difference-of-arrival}
\newacro{aoa}[AOA]{angle-of-arrival}
\newacro{rss}[RSS]{received signal strength}


\newacro{crb}[CRB]{Cram\'{e}r-Rao Bound}
\newacro{speb}[SPEB]{squared position error bound}
\newacro{fim}[FIM]{Fisher information matrix}
\newacro{pocs}[POCS]{projection onto convex sets}


\newacro{eed}[EED]{Engineering Every Day}
\newacro{stem}[STEM]{science, technology, engineering, and mathematics}

\newacro{LOCC}[LOCC]{local operations and classical communication}
\newacro{ebit}[ebit]{entanglement bit}
\newacro{NISQ}[NISQ]{Noisy Intermediate-Scale Quantum}
\newacro{CDF}[CDF]{Cumulative Distribution Function}
\newacro{QSD}[QSD]{Quantum State Discrimination}

\newacro{PPT}[PPT]{positive partial transposition} 


